Directly finite algebras of pseudofunctions on locally compact groups

An algebra $A$ is said to be directly finite if each left invertible element in the (conditional) unitization of $A$ is right invertible. We show that the reduced group ${\rm C}^\ast$-algebra of a unimodular group is directly finite, extending known results for the discrete case. We also investigate the corresponding problem for algebras of $p$-pseudofunctions, showing that these algebras are directly finite if $G$ is amenable and unimodular, or unimodular with the Kunze--Stein property. An exposition is also given of how existing results from the literature imply that $L^1(G)$ is not directly finite when $G$ is the affine group of either the real or complex line.

==> df-pfp_mac.tex <==

\NeedsTeXFormat{LaTeX2e}
\RequirePackage{amsmath,amssymb,amsfonts}
%\usepackage{YCmath,YCthm,abbrev}

\usepackage[usenames]{color}

\setlength{\textwidth}{\paperwidth}
\addtolength{\textwidth}{-65mm}
\setlength{\oddsidemargin}{6mm}
\setlength{\evensidemargin}{6mm}
\setlength{\topmargin}{0mm}

\setlength{\textheight}{\paperheight}
\addtolength{\textheight}{-65mm}

\NeedsTeXFormat{LaTeX2e}
% load up Paul Taylor's diagram.sty macros
%\RequirePackage[UglyObsolete]{diagrams}
% noPostScript option invoked to avoid annoying rotation of diagonal labels
\RequirePackage[PS,nohug]{diagrams}


\newcommand{\dt}[1]{\textcolor{Maroon}{\textsf{#1}}}
\newcommand{\st}{\;:\;}

\newcommand{\defeq}{:=}
\renewcommand{\emph}[1]{{\sl #1}\/} % use slanted font for emphasis

% journals seem to want upright roman numerals in numbered lists, we need to force this if in an italic environment
\newenvironment{YCnum}{%
\begin{enumerate}
\renewcommand{\labelenumi}{{\rm(\roman{enumi})}}
\renewcommand{\theenumi}{{\rm(\roman{enumi})}}
}{\end{enumerate}\ignorespacesafterend}


\newcommand{\bbF}{{\mathbb F}}
\newcommand{\Real}{{\mathbb R}}
\newcommand{\Cplx}{\mathbb C}
\newcommand{\Bdd}{{\mathcal B}}
\newcommand{\Cpct}{{\mathcal K}}
\newcommand{\veps}{\varepsilon}
\newcommand{\supp}{\operatorname{supp}}

\newcommand{\fu}[1]{{#1}^{\sharp}}    % forced unitisation
                % Helemskii denotes this by A_+, etc.
\newcommand{\cu}[1]{{#1}_{\rm un}}  % conditional unitisation
\newcommand{\id}[1][]{{\sf 1}_{#1}} % identity of group, algebra, object in category

\newcommand{\abs}[1]{\vert{#1}\vert}
\newcommand{\Abs}[1]{\left\vert{#1}\right\vert}
\newcommand{\bigabs}[1]{\bigl\vert{#1}\bigr\vert} % needs amsmath?
\newcommand{\norm}[1]{\Vert{#1}\Vert}
\newcommand{\Norm}[1]{\left\Vert{#1}\right\Vert}
\newcommand{\xnorm}[2]{\left\Vert#1\right\Vert_{(#1)}}

\newcommand{\tp}{\mathrel{\otimes}}
\newcommand{\ptp}{\mathrel{\widehat{\otimes}}}

%%% Fourier algebra, von Neumann algebra, etc
\newcommand{\PF}{\operatorname{PF}}
\newcommand{\PM}{\operatorname{PM}}
\newcommand{\CV}{\operatorname{CV}}
\newcommand{\VN}{\operatorname{VN}}
\newcommand{\FA}{\operatorname{A}}
\newcommand{\Cst}{\ensuremath{\operatorname{C}^*}}
\newcommand{\SIN}{\ensuremath{\operatorname{SIN}}}
\newcommand{\SL}{\operatorname{SL}}
\newcommand{\FIN}{\operatorname{FIN}}
%-------------

\newcommand{\Aff}{\operatorname{Aff}} % Affine groups
\newcommand{\Caff}{\Aff(\Cplx)}
\newcommand{\Raff}{\Aff(\Real)}

\newcommand{\ran}{\operatorname{ran}}
\newcommand{\qm}{\mathrel{\bullet}} % quasi-multiplication

\renewcommand{\Re}{\operatorname{Re}}

\newcommand{\cA}{{\mathcal A}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cM}{{\mathcal M}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\fA}{{\mathfrak A}}
\newcommand{\fB}{{\mathfrak B}}
%\newcommand{\fg}{{\mathfrak g}}
\newcommand{\fH}{{\mathfrak H}}
\newcommand{\fm}{{\mathfrak m}}
\newcommand{\fn}{{\mathfrak n}}
\newcommand{\sL}{{\sf L}}
\newcommand{\sR}{{\sf R}}
\newcommand{\sS}{{\sf S}}

%\newcommand{\ip}[2]{(#1\vert#2)}

%\newcommand{\YCrem}[1]{\textbf{(\textit{#1} -- YC)}}


\newcommand{\al}{\alpha}
\newcommand{\lm}{\lambda}
\newcommand{\Gm}{\Gamma}

\newcommand{\pair}[2]{\langle#1,#2\rangle}

\newcommand{\qdf}{directly finite}  % alias, probably phase out in final version

\newcommand{\dual}[1]{\widehat{#1}}


\newcounter{pulse}[section]
\numberwithin{pulse}{section}  % all thms, etc set from pulse

\usepackage{amsthm}
%Styles for theorems, definitions, remarks

%-Theorems
\theoremstyle{plain}
\newtheorem{thm}[pulse]{\sc Theorem}
\newtheorem{prop}[pulse]{\sc Proposition}
\newtheorem{lem}[pulse]{\sc Lemma}
\newtheorem{cor}[pulse]{\sc Corollary}
\newtheorem{qu}{\sc Question}
%-Definitions
\theoremstyle{definition}
\newtheorem{dfn}[pulse]{\sc Definition}
\newtheorem*{notn}{\sc Notation}
\newtheorem{eg}[pulse]{\sc Example}
%-Remarks
\theoremstyle{remark}
\newtheorem{rem}[pulse]{\sc Remark}
\newtheorem*{remstar}{\sc Remark}
\newtheorem{egs}[pulse]{Examples}

%\newcommand{\Mat}[1]{{\mathbb M}_{#1}}
\newcommand{\ip}[2]{\langle#1,#2\rangle}
\newcommand{\adj}{\operatorname{adj}} %adjugate

\renewcommand{\ip}[2]{(#1\mid#2)}
\newcommand{\dotvphi}{\dot{\varphi}}

\newcommand{\twomat}[4]{\left(\begin{matrix}#1 & #2 \\ #3 & #4 \end{matrix}\right)}


\newcommand{\iso}{\cong}
\newcommand{\tilimath}{\widetilde{\imath}}
%
\newcommand{\tillm}{\widetilde{\lambda}}
\newcommand{\LplusPG}[1]{{L^{#1}(G) \oplus_1 \PF_{#1}(G)}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\iKS}{\imath_{\rm KS}}
\newcommand{\Aut}{\operatorname{Aut}}
\newcommand{\wstar}{\ensuremath{\operatorname{w}^*}}
%

